Memory-efficient particle filter recurrent neural network for object localization

This study proposes a novel memory-efficient recurrent neural network (RNN) architecture specified to solve the object localization problem. This problem is to recover the object states along with its movement in a noisy environment. We take the idea of the classical particle filter and combine it with GRU RNN architecture. The key feature of the resulting memory-efficient particle filter RNN model (mePFRNN) is that it requires the same number of parameters to process environments of different sizes. Thus, the proposed mePFRNN architecture consumes less memory to store parameters compared to the previously proposed PFRNN model. To demonstrate the performance of our model, we test it on symmetric and noisy environments that are incredibly challenging for filtering algorithms. In our experiments, the mePFRNN model provides more precise localization than the considered competitors and requires fewer trained parameters.

==> 05-conclusion.tex <==
\section{Conclusion}

We present the novel recurrent neural network architecture mePFRNN to solve the object localization problem.
It combines the standard GRU RNN, particle filter, and explicit measurements of distances from the object to the beacons.
The latter feature makes the proposed model memory-efficient since the number of trainable parameters does not depend on the environment size.
% Also, the proposed mePFRNN is specifically important for the localization problem and is not essential for stock prediction or any other applications dealing with sequential data addressed by the PFRNN model.
We compare the proposed mePFRNN model with the general-purpose PFRNN model and two modifications of standard GRU RNN.
The test environments consist of symmetric environments of different sizes and the non-symmetric \emph{Labyrinth} environment.
Such diversity of the test environments leads to the comprehensive comparison of the considered parametric models to solve the object localization problem.
% Although mePFRNN appears slightly slower in inference than the baseline PFRNN, it filters the object's coordinates much more precisely in the considered symmetric environments.
Although mePFRNN appears slightly slower in inference than the baseline PFRNN, it filters the object's coordinates more precisely in the considered symmetric environments.
Moreover, mePFRNN does not exploit explicit data about the environment or the corresponding embeddings.
At the same time, the proposed mePFRNN model outperforms competitors in MSE values for the most of considered test environments.


